Section Patterns: Efficiently Solving Narrow Passage Problems in Multilevel Motion Planning

Sampling-based planning methods often become inefficient due to narrow passages. Narrow passages induce a higher runtime, because the chance to sample them becomes vanishingly small. In recent work, we showed that narrow passages can be approached by relaxing the problem using admissible lower-dimensional projections of the state space. Those relaxations often increase the volume of narrow passages under projection. Solving the relaxed problem is often efficient and produces an admissible heuristic we can exploit. However, given a base path, i.e. a solution to a relaxed problem, there are currently no tailored methods to efficiently exploit the base path. To efficiently exploit the base path and thereby its admissible heuristic, we develop section patterns, which are solution strategies to efficiently exploit base paths in particular around narrow passages. To coordinate section patterns, we develop the pattern dance algorithm, which efficiently coordinates section patterns to reactively traverse narrow passages. We combine the pattern dance algorithm with previously developed multilevel planning algorithms and benchmark them on challenging planning problems like the Bugtrap, the double L-shape, an egress problem and on four pregrasp scenarios for a 37 degrees of freedom shadow hand mounted on a KUKA LWR robot. Our results confirm that section patterns are useful to efficiently solve high-dimensional narrow passage motion planning problems.

==> images/figure_fiberbundle.tex <==
\begin{figure}
    \centering
\resizebox{0.8\linewidth}{!}{

\begin{tikzpicture}
\def\height{2}
\def\radius{1.25}
\def\heightEllipse{0.5}
\def\distBase{1.8}
\def\pathLength{1.5}
\def\vertexStart{-0.5*\pathLength}
\def\pathStretch{2*3.1415/\pathLength}

\def\xposFiber{-2.5*\radius}
\def\xposPath{0*\radius}
%\def\xposGraph{2.2*\radius}

\tikzset{
    classical/.style={thin,double,->,shorten >=4pt,shorten <=4pt,>=stealth}
}
\newcommand\drawCylinder[1]{
\draw (#1,\height) ellipse ({\radius} and \heightEllipse);
\draw (#1-\radius,0) -- (#1-\radius,\height);
\draw (#1+\radius,0) -- (#1+\radius,\height);
\draw (#1-\radius,0) arc (180:360:{\radius} and \heightEllipse);
\draw [dashed] (#1-\radius,0) arc (180:360:{\radius} and -\heightEllipse);
\draw (#1,-\distBase) ellipse ({\radius} and \heightEllipse);
\draw[classical] (#1,0-\heightEllipse) -- (#1,-\distBase+\heightEllipse);
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Draw Path
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\ppath[1]{
0.13*sin(180*(\pathStretch*(#1-\pathStart))/3.14)
}
\newcommand\drawPath[1]{
\def\pathStart{#1+\vertexStart}
\draw plot [smooth,samples=10,domain=\pathStart:{\pathStart+\pathLength}](\x,{\ppath{\x} - \distBase});
\fill [gray, pattern=vertical lines, opacity=0.8]
plot [smooth,samples=10,domain=\pathStart:{\pathStart+\pathLength}](\x,{\ppath{\x}}) -- 
plot [smooth,samples=10,domain={\pathStart+\pathLength}:\pathStart](\x,{\ppath{\x} + \height});

\foreach \y in {0,0.5,...,\height}
\draw plot [smooth,samples=10,domain=\pathStart:{\pathStart+\pathLength}](\x,{\ppath{\x} + \y});

\draw (\pathStart,0) -- (\pathStart, \height);
\draw (\pathStart+\pathLength,0) -- (\pathStart+\pathLength, \height);
}

\newcommand\drawFiber[1]{
\def\pointPosX{#1+0.5*\radius}
\draw[line width=0.3mm,black](\pointPosX,0) -- (\pointPosX, \height);
\node[draw,fill,circle,inner sep=0pt,minimum size=0.3mm] at (\pointPosX, 0-\distBase){};
\draw node[left] at (\pointPosX, 0-\distBase) {$x_B$};
\draw node[left] at (\pointPosX, 0.5*\height) {$\pi^{-1}(x_B)$};
}

\newcommand\drawGraphCC[2]{
\draw 
(#1+\vertexStart+1.2*\pathLength,#2 - 0.1*\heightEllipse)
-- (#1+\vertexStart+0.9*\pathLength,#2 + 0.3*\heightEllipse)
-- (#1+\vertexStart+0.6*\pathLength,#2 + 0.5*\heightEllipse)
-- (#1+\vertexStart+0.4*\pathLength,#2 - 0.5*\heightEllipse)
-- (#1+\vertexStart+0.75*\pathLength,#2 - 0.4*\heightEllipse)
-- (#1+\vertexStart+0.9*\pathLength,#2 + 0.3*\heightEllipse);
}


\tikzset{
  vertex/.style = {shape=circle,inner sep=0,outer sep=0},
  edge/.style = {->,-Latex},
}
\node[vertex] (a) at (+\vertexStart+1.2*\pathLength, - 0.1*\heightEllipse) {};
\node[vertex] (b) at (+\vertexStart+0.9*\pathLength, + 0.3*\heightEllipse) {};
\node[vertex] (c) at (+\vertexStart+0.6*\pathLength, + 0.5*\heightEllipse) {};
\node[vertex] (d) at (+\vertexStart+0.4*\pathLength, - 0.5*\heightEllipse) {};
\node[vertex] (e) at (+\vertexStart+0.75*\pathLength, - 0.4*\heightEllipse) {};
\node[vertex] (f) at (+\vertexStart+0.9*\pathLength, + 0.3*\heightEllipse) {};

\node[vertex] (g) at (+\vertexStart-0.2*\pathLength, -0.2*\heightEllipse) {};
\node[vertex] (h) at (+\vertexStart+0.2*\pathLength, + 0.1*\heightEllipse) {};
\node[vertex] (i) at (+\vertexStart+0.05*\pathLength, + 0.5*\heightEllipse) {};

\def\edgeList{a/b, b/c, c/d, d/e, e/b, g/h, h/i, i/g}

\newcommand\drawGraph[2]{
\foreach \source/\target in \edgeList
    \draw ($(\source)+(#1,#2)$) -- 
    ($(\target)+(#1,#2)$);
}
\newcommand\drawGraphRestriction[3]{
\foreach \source/\target in \edgeList
    \fill [gray, draw, pattern=vertical lines, opacity=0.8]
    ($(\source)+(#1,#2)$) -- 
    ($(\target)+(#1,#2)$) --
    ($(\target)+(#1,#2)+(0,#3)$) --
    ($(\source)+(#1,#2)+(0,#3)$) --
    ($(\source)+(#1,#2)$);
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\drawCylinder{\xposFiber}
\drawFiber{\xposFiber}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\drawCylinder{\xposPath}
\drawPath{\xposPath}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\drawGraph{\xposGraph}{-\distBase}
%\foreach \y in {0,0.5,...,\height}
%   \drawGraph{\xposGraph}{\y};
%\drawCylinder{\xposGraph}
%\drawGraphRestriction{\xposGraph}{0}{\height};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\end{tikzpicture}
}
    \caption{Bundle restrictions on fiber bundle $\R^3 \rightarrow \R^2$. Left: Point restriction (Fiber). Right: Path restriction over base path. Taken from \cite{Orthey2020IJRR}.\label{fig:fiberbundle}}
\end{figure}

==> images/figure_pull.tex <==
\begin{figure}[ht]
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/pullfigure/P1.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/pullfigure/P2.png}
    \end{subfigure}
    
    \begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/pullfigure/P4.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/pullfigure/P3.png}
    \end{subfigure}
    
    \begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/pullfigure/P5.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/pullfigure/P6.png}
    \end{subfigure}
\caption{\label{fig:limitations}}
\end{figure}
